Distributed Processing for Encoding and Decoding of Binary LDPC codes using MPI

Low Density Parity Check (LDPC) codes are linear error correcting codes used in communication systems for Forward Error Correction (FEC). But, intensive computation is required for encoding and decoding of LDPC codes, making it difficult for practical usage in general purpose software based signal processing systems. In order to accelerate the encoding and decoding of LDPC codes, distributed processing over multiple multi-core CPUs using Message Passing Interface (MPI) is performed. Implementation is done using Stream Processing and Batch Processing mechanisms and the execution time for both implementations is compared w.r.t variation in number of CPUs and number of cores per CPU. Performance evaluation of distributed processing is shown by variation in execution time w.r.t. increase in number of processors (CPU cores).

==> Demo_Proposal.tex <==
\newpage
%\onecolumn
\section{Demo Proposal}\label{sec:demo}

To perform encoding and decoding of LDPC codes, a MPI C++ library consisting of various functions has been created. Functions such as creation of Parity Check matrix, creation of Generator matrix, encoding with stream processing and batch processing, decoding with stream processing and batch processing, etc. The usage of various functions will be shown for the demo. The functions have been created with the purpose of using LDPC codes for experiments in any inter-connected CPU cluster with an MPI based compiler for C++. Any Binary Parity Check matrix or Generator matrix created using other applications can be used for encoding and decoding using this library. The main functionality for decoding is to create an a bipartite graph using the Parity Check matrix and performing Sum-Product decoding using the graph. Also, for encoding the library converts the Generator Matrix to standard form and then uses it to encode input information bits.

For the demo, the encoding and decoding processes of LDPC codes will be performed. Two types of demos will be performed. For both the demos, execution will be first done on a single server, consisting of multiple CPUs and then on 2 servers each having multiple CPUs. Each CPU will consist of multiple cores. For each demo, Stream processing and Batch processing will be performed, and the execution time for both will be displayed and compared.

For the first demo, the code length will be kept constant, and the rate of LDPC code will be varied. For each rate selected, the number of processors to be used will be increased from 1 to maximum number of logical cores present in the combined set of CPUs used. 
